ISP: Multi-Layered Garment Draping with Implicit Sewing Patterns

Many approaches to draping individual garments on human body models are realistic, fast, and yield outputs that are differentiable with respect to the body shape on which they are draped. However, they are either unable to handle multi-layered clothing, which is prevalent in everyday dress, or restricted to bodies in T-pose. In this paper, we introduce a parametric garment representation model that addresses these limitations. As in models used by clothing designers, each garment consists of individual 2D panels. Their 2D shape is defined by a Signed Distance Function and 3D shape by a 2D to 3D mapping. The 2D parameterization enables easy detection of potential collisions and the 3D parameterization handles complex shapes effectively. We show that this combination is faster and yields higher quality reconstructions than purely implicit surface representations, and makes the recovery of layered garments from images possible thanks to its differentiability. Furthermore, it supports rapid editing of garment shapes and texture by modifying individual 2D panels.

==> figs/ablation.tex <==
\begin{figure}[t]
	\centering
		\begin{minipage}{.4\textwidth}
				\centering
		% \vspace{1mm}
		\includegraphics[width=.99\textwidth]{figs/normal_p.pdf}
		% \vspace{-7mm}
		\captionof{figure}{\textbf{Ablation on $\mathcal{L}_{normal}$}. Training without it yields flipped triangle faces (shown in dark grey).}
		\label{fig:normal}
	\end{minipage}
	% \hspace{0mm}
	\begin{minipage}{.57\textwidth}
		\centering
		\includegraphics[width=.99\textwidth]{figs/consist_p.pdf}
		% \vspace{-10pt}
		\captionof{figure}{\textbf{Ablation on $\mathcal{L}_{consist}$}. The skirts reconstructed by the models trained (a) with $\mathcal{L}_{consist}$ and (b) without $\mathcal{L}_{consist}$. The latter has a gap between its front and back panels.}
		\label{fig:consist}
	\end{minipage}%
	% \vspace{-6mm}
\end{figure}

==> figs/consist.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/consist_p.pdf}
    %\vspace{-0.35cm}
    \caption{consist.}
    \label{fig:consist}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/failure.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/failure_p.pdf}
    %\vspace{-0.35cm}
    \caption{Draping increasingly many shirts: from 1 (left) to 7 (right).}
    \label{fig:failure}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/interp.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/interp_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Interpolation}. We interpolate the latent code from a sleeveless shirt to a long-sleeve jacket. (a) and (b) show the reconstructed front and back panels, where the colors on them denote the edge label fields. (c) shows the reconstructed mesh.}
    \label{fig:interp}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/normal.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/normal_p.pdf}
    %\vspace{-0.35cm}
    \caption{Recon.}
    \label{fig:normal}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/pip.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figs/pip_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Framework of our approach}. \textbf{Top}: For the garment representation, we train an the implicit network $\mathcal{I}_{\Theta}$ to predict the signed distance field ($s_f$/$s_b$) and the edge label field ($c_f$/$c_b$) that represent front and back 2D panels.
    Together, they form the garment sewing pattern.
    The rest-state garment mesh is reconstructed by mapping the patterns to 3D space via the UV parameterization network $\mathcal{A}_{\Phi}$. \textbf{Bottom}: Garment draping. We first apply the network $\mathcal{D}_s$ to drape single garments. By utilizing the garment geometry and forces encoded in the input UV maps, we then rely on the network $\mathcal{D}_m$ to resolve garment intersections for multi-layered draping.}
    \label{fig:pip}
    %\vspace{-0.45cm}
\end{figure} 


==> figs/supp_6_panels.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_6_panels_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{The 6-panel sewing pattern}. (a) The 3D mesh surface for a shirt. The corresponding surface for each panel is denoted in different colors. (b) The six 2D panels for the front, the back, the right front/back sleeves and the left front/back sleeves.}
    \label{fig:supp_6_panels}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_6_panels_recon.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_6_panels_recon_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Reconstruction with 6 panels}. For both the left and right examples, we show the reconstructed panels on the top and the reconstructed surfaces and the sewed meshes at the bottom. Colors on panels denote edge labels predicted by $\mathcal{I}_{\Theta}$.}
    \label{fig:supp_6_panels_recon}
\end{figure} 

==> figs/supp_arch.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/supp_arch_p.pdf}
    %\vspace{-0.35cm}
    \caption{The architecture of the pattern parameterization network $\mathcal{I}_{\Theta}$.}
    \label{fig:supp_arch}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_atlas.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_atlas_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Comparison with AtlasNet}. The meshes in black boxes are the source patches where the mapping function is applied: a square patch for AtlastNet, a garment panel for our method.}
    \label{fig:supp_atlas}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_dig_snug_ours.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_dig_snug_ours_p.pdf}
    %\vspace{-0.35cm}
    \caption{The comparison of draping results for (a) our method vs. DIG, and (b) our method vs. SNUG.}
    \label{fig:supp_dig_snug_ours}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_drapenet_ours.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_drapenet_ours_p.pdf}
    %\vspace{-0.35cm}
    \caption{The comparison of draping results of our method and DrapeNet.}
    \label{fig:supp_drapenet_ours}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_heatmap.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figs/supp_heatmap_p.pdf}
    \caption{\textbf{Comparative analysis of mesh reconstruction and spatial error distribution for shirt, skirt and trousers}. (a) represents the ground truth mesh. (b) and (d) illustrate the mesh reconstruction and corresponding spatial error distribution for our proposed method. (c) and (e) display the same for UDFs. Each row provides both front (upper half) and back (lower half) views. In (d) and (e), error magnitude is indicated by color gradation, with white representing large errors and blue small errors.}
    \label{fig:supp_heatmap}
\end{figure} 


==> figs/supp_interp_pants.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_interp_pants_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Interpolation}. We interpolate the latent code from a pair of short trousers to a pair of long trousers. (a) and (b) show the reconstructed front and back panels, where the colors on them denote the edge label fields. (c) shows the reconstructed mesh.}
    \label{fig:supp_interp_pants}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_interp_skirt.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_interp_skirt_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Interpolation}. We interpolate the latent code from a short tight skirt to a long loose skirt. (a) and (b) show the reconstructed front and back panels, where the colors on them denote the edge label fields. (c) shows the reconstructed mesh.}
    \label{fig:supp_interp_skirt}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_layer.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/supp_layer_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Ablation on layering.} We first drape a red and a orange shirts on the body (a), then a third one (yellow) is draped by the Algorithm \ref{alg:mld} (b) and the one-step algorithm (c).}
    \label{fig:supp_layer}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_mesh.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_mesh_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Meshing Process.} Starting with a square 2D mesh $\mathbf{T}$, we first extract the front and back panel meshes $\mathbf{T}_{P_f}$ and $\mathbf{T}_{P_b}$ using the implicit function $\mathcal{I}_{\Theta}$. Then we lift $\mathbf{T}_{P_f}$ and $\mathbf{T}_{P_b}$ to 3D to get the surface meshes $\mathbf{T}_{S_f}$ and $\mathbf{T}_{S_b}$ by querying $\mathcal{A}_{\Phi_f}$ and $\mathcal{A}_{\Phi_b}$ on their vertices respectively.}
    \label{fig:supp_mesh}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_pattern.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_pattern_p.pdf}
    %\vspace{-0.35cm}
    \caption{The sewing patterns for (a) trousers and (b) skirts. The front mesh surfaces are in gray and the back ones in blue.}
    \label{fig:supp_pattern}
    %\vspace{-0.45cm}
  \end{figure} 

==> figs/supp_pipD.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
	\centering
		\begin{minipage}{.40\textwidth}
				\centering
		% \vspace{1mm}
		\includegraphics[width=0.99\textwidth]{figs/supp_pipD2_p.pdf}
		% \vspace{-7mm}
		\captionof{figure}{\textbf{Single layer draping.} The rest-state garment is first deformed by the diffused LBS to get the initial shape, and then refined by the displacement maps predicted by $\mathcal{D}_s$. }
		\label{fig:supp_pipD}
	\end{minipage}
	% \hspace{0mm}
    ~
	\begin{minipage}{.58\textwidth}
		\centering
		\includegraphics[width=.99\textwidth]{figs/supp_layer_p.pdf}
		% \vspace{-10pt}
		\captionof{figure}{\textbf{Layering.} (a) We drape a red and an orange shirts on the body. A third one (yellow) is draped by (b) Algorithm \ref{alg:mld} and (c) by naively applying $\mathcal{D}_m$ to it.}
		\label{fig:supp_layer}
	\end{minipage}%
    \vspace{-0.45cm}
\end{figure}


\iffalse
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_pipD_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{The pipeline of garment draping}. We first apply the network $\mathcal{D}_s$ to drape single garments. By utilizing the garment geometry and forces encoded in the input UV maps, we then rely on the network $\mathcal{D}_m$ to resolve garment intersections for multi-layered draping.}
    \label{fig:supp_pipD}
    %\vspace{-0.45cm}
\end{figure} 
\fi

==> figs/supp_recon_pants.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_recon_pants_p.pdf}
    %\vspace{-0.35cm}
    \caption{Reconstruction samples of trousers.}
    \label{fig:supp_recon_pants}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_recon_shirt.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_recon_shirt_p.pdf}
    %\vspace{-0.35cm}
    \caption{Reconstruction samples of shirts.}
    \label{fig:supp_recon_shirt}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_recon_skirt.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_recon_skirt_p.pdf}
    %\vspace{-0.35cm}
    \caption{Reconstruction samples of skirts.}
    \label{fig:supp_recon_skirt}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_seg.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/supp_seg_p.pdf}
    %\vspace{-0.35cm}
    \caption{Segmentation masks obtained from \cite{Li20i}. Jackets are marked in gray, shirts in purple, skirts in dark purple, trousers in red, and body parts in other colors.}
    \label{fig:supp_seg}
    %\vspace{-0.45cm}
\end{figure} 

==> figs/supp_sew.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/supp_sew3_p.pdf}
  %\vspace{-0.35cm}
  \caption{\textbf{Sewing process.} Left: the boundary vertices belonging to the sewing edges $E_c^f$ and $E_c^b$ are marked in red. Middle: The triangulation is performed between $E_c^f$ and $E_c^b$ to create new faces $F_{sew}$. Right: The mesh generated by merging the front and back surfaces $\mathbf{T}_{S_f}$ and $\mathbf{T}_{S_b}$ with $F_{sew}$.}
  \label{fig:supp_sew}
  %\vspace{-0.45cm}
\end{figure} 


==> figs/texture.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/texture_p.pdf}
    %\vspace{-0.35cm}
    \caption{\textbf{Texture editing.}
    \textbf{(a)} A smiling face drawn on the front panel.
    \textbf{(b)} A flower pattern painted on both the front and the back panels.  
    \textbf{(c)} A pocket drawn for the left shirt can be transferred to different garments.}
    \label{fig:texture}
    %\vspace{-0.45cm}
\end{figure} 

==> tabs/collisions.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[h!]
  \begin{center}
  \scalebox{0.8}{
    \begin{tabular}{c | c | c | c | c | c}
      \toprule
       w/ $\mathcal{D}_m$ & 1 & 2 & 3 & 4 & 5 \\
       \midrule
       1  & 0.000 & 0.067 & 0.001 & 0.000 & 0.000 \\
       2  & - & 0.003 & 0.633 & 0.608 & 0.636 \\
       3  & - & - & 0.028 & 1.224 & 1.158 \\
       4  & - & - & - & 0.019 & 2.449\\
       5  & - & - & - & - & 0.035 \\
      \bottomrule
      \end{tabular}}
      ~~
  \scalebox{0.8}{
    \begin{tabular}{c | c | c | c | c | c}
      \toprule
       w/o $\mathcal{D}_m$ & 1 & 2 & 3 & 4 & 5 \\
       \midrule
       1  & 0.000 & 0.456 & 0.340 & 0.357 & 0.233 \\
       2  & - & 0.004 & 28.033 & 26.378 & 26.246 \\
       3  & - & - & 0.046 & 24.729 & 24.679 \\
       4  & - & - & - & 0.073 & 27.821\\
       5  & - & - & - & - & 0.052 \\
      \bottomrule
      \end{tabular}}
  \end{center}
  \caption{Evaluation of intersections with the underlying body and between garments on different layers (the 1st layer is a \textbf{skirt}). Left and right are the results of draping with and without the multi-layering network $\mathcal{D}_m$, respectively. The unit is \%.}
  \label{tab:collisions_skirt}
\end{table}


\begin{table}[h!]
  \begin{center}
  \scalebox{0.8}{
    \begin{tabular}{c | c | c | c | c | c}
      \toprule
       w/ $\mathcal{D}_m$ & 1 & 2 & 3 & 4 & 5 \\
       \midrule
       1  & 0.185 & 0.048 & 0.000 & 0.000 & 0.000 \\
       2  & - & 0.003 & 0.631 & 0.588 & 0.637 \\
       3  & - & - & 0.030 & 1.227 & 1.161 \\
       4  & - & - & - & 0.020 & 2.426\\
       5  & - & - & - & - & 0.028 \\
      \bottomrule
      \end{tabular}}
      ~~
  \scalebox{0.8}{
    \begin{tabular}{c | c | c | c | c | c}
      \toprule
       w/o $\mathcal{D}_m$ & 1 & 2 & 3 & 4 & 5 \\
       \midrule
       1  & 0.185 & 0.225 & 0.259 & 0.223 & 0.134 \\
       2  & - & 0.004 & 28.033 & 26.378 & 26.246 \\
       3  & - & - & 0.046 & 24.729 & 24.679 \\
       4  & - & - & - & 0.073 & 27.821\\
       5  & - & - & - & - & 0.052 \\
      \bottomrule
      \end{tabular}}
  \end{center}
  \caption{Evaluation of intersections with the underlying body and between garments on different layers (the 1st layer is a pair of \textbf{trousers}). Left and right are the results of draping with and without the multi-layering network $\mathcal{D}_m$, respectively. The unit is \%.}
  \label{tab:collisions_trousers}
\end{table}

==> tabs/intersection.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US
%\begin{wraptable}{r}{4.5cm}
\begin{table}
  \begin{center}
    \scalebox{.8}{
          \begin{tabular}{c | c}
          \toprule
             & Intersection (\%, $\downarrow$)\\
           \midrule
           DrapeNet  & 0.536  \\
           Ours  & \textbf{0.276}  \\
          \bottomrule
          \end{tabular}
          }
    \end{center}
    \vspace{-0.2cm}
    \caption{Comparison between DrapeNet and our method for shirts and trousers on the ratio of intersection areas (Intersection).
    }
    \label{tab:intersection}
    %\vspace{-6mm}
    %\vspace{-0.5cm}
\end{table}
%\end{wraptable} 


==> tabs/normal.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \begin{center}
    \scalebox{1.}{
          \begin{tabular}{c | c | c }
          \toprule
             & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$)\\
           \midrule
           w/o $\mathcal{L}_{normal}$  & 0.324 & 98.69  \\
           w/ $\mathcal{L}_{normal}$  & 0.321 & 99.08  \\
          \bottomrule
          \end{tabular}
          }
    \end{center}
    %\vspace{-0.5cm}
    \caption{Comparison of the results reconstructed by the models trained w/o and w/ $\mathcal{L}_{normal}$.
    }
    \label{tab:normal}
    %\vspace{-6mm}
\end{table}


==> tabs/parameters.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US
  
\begin{table}
    \begin{center}
        \begin{tabular}{c|cc|cc|ccc}
        \toprule
        \multirow{2}{*}{Loss} &
            \multicolumn{2}{c|}{$\mathcal{L}_{\mathcal{I}}$} &
            \multicolumn{2}{c|}{$\mathcal{L}_{\mathcal{A}}$} &
            \multicolumn{3}{c}{$\mathcal{L}_{\mathcal{D}_m}$} \\
            & $\lambda_{CE}$ & $\lambda_{reg}$ & $\lambda_{n}$ & $\lambda_{c}$ & $\lambda_{g}$ & $\lambda_{r}$ & $\epsilon$ \\
            \midrule
        Value & 0.01 & 0.001 & 0.01 & 1 & 0.5 & 1 & 0.005 \\
        \bottomrule
        \end{tabular}
    \end{center}
    \caption{Training loss hyperparameters for $\mathcal{L}_{\mathcal{I}}$, $\mathcal{L}_{\mathcal{A}}$ and $\mathcal{L}_{\mathcal{D}_m}$.
    }
    \label{tab:parameters}
\end{table}

==> tabs/recon_pants.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
    \begin{center}
      \scalebox{1.}{
            \begin{tabular}{c | c | c | c}
            \toprule
             Trousers & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) & Time (ms, $\downarrow$) \\
             \midrule
             UDF - 128  & 0.758 & 98.22 & 661 \\
             UDF - 256  & 0.430 & 98.56 & 2650 \\
             UDF - 512  & 0.342 & 98.33 & 17141 \\
             \midrule
             Ours - 128  & 0.545 & 98.28 & \textbf{25} \\
             Ours - 256  & 0.363 & 98.59 & 82 \\
             Ours - 512  & \textbf{0.317} & \textbf{98.62} & 269 \\
            \bottomrule
            \end{tabular}
            }
      \end{center}
      %\vspace{-0.5cm}
      \caption{Comparison of our method to UDF \cite{DeLuigi23} on trousers under the resolutions of 128, 256 and 512.
      }
      \label{tab:recon_pants}
      %\vspace{-6mm}
      %\vspace{-0.5cm}
  \end{table}
  

==> tabs/recon_skirt.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%\begin{table}
%    \begin{center}
%      \scalebox{1.}{
%            \begin{tabular}{c | c | c | c}
%            \toprule
%             Skirt & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) & Time (ms, $\downarrow$) \\
%             \midrule
%             UDF - 128  & 0.714 & 98.53 & 690 \\
%             UDF - 256  & 0.408 & 98.93 & 2784 \\
%             UDF - 512  & 0.331 & 98.43 & 17362 \\
%             \midrule
%             Ours - 128  & 0.538 & 98.80 & \textbf{25} \\
%             Ours - 256  & 0.321 & 99.08 & 75 \\
%             Ours - 512  & \textbf{0.267} & \textbf{99.14} & 262 \\
%            \bottomrule
%            \end{tabular}
%            }
%      \end{center}
      %\vspace{-0.5cm}
%      \caption{Comparison of our method to UDF \cite{DeLuigi23} on skirts under the resolutions of 128, 256 and 512.
%      }
%      \label{tab:recon_skirt}
      %\vspace{-6mm}
      %\vspace{-0.5cm}
%  \end{table}
  
\begin{table}[h!]
  \begin{center}
  \scalebox{0.75}{
    \begin{tabular}{c | c | c | c}
      \toprule
       Train & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) & Time (ms, $\downarrow$) \\
       \midrule
       UDF - 128  & 0.714 & 98.53 & 690 \\
       UDF - 256  & 0.408 & 98.93 & 2784 \\
       UDF - 512  & 0.331 & 98.43 & 17362 \\
       \midrule
       Ours - 128  & 0.538 & 98.80 & \textbf{25} \\
       Ours - 256  & 0.321 & 99.08 & 75 \\
       Ours - 512  & \textbf{0.267} & \textbf{99.14} & 262 \\
      \bottomrule
      \end{tabular}}
      ~~
  \scalebox{0.75}{
    \begin{tabular}{c | c | c}
      \toprule
       Test & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) \\
       \midrule
       UDF - 128  & 0.734 & 97.79 \\
       UDF - 256  & 0.403 & 98.64 \\
       UDF - 512  & 0.324 & 98.27 \\
       \midrule
       Ours - 128  & 0.583 & 98.62 \\
       Ours - 256  & 0.362 & 98.85 \\
       Ours - 512   & \textbf{0.304} & \textbf{98.89} \\
      \bottomrule
      \end{tabular}
    }
  \end{center}
  \vspace{-1mm}
  \caption{Comparison of our method to UDF on skirts under the resolutions of 128, 256 and 512.}
  \vspace{-4.5mm}
  \label{tab:recon_skirts}
\end{table}


==> tabs/recon_unseen.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
    \begin{center}
      \scalebox{1.}{
            \begin{tabular}{c | c | c}
            \toprule
             Shirt & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) \\
             \midrule
             UDF  & 0.493 & 98.44 \\
             \midrule
             Ours  & \textbf{0.392} & \textbf{98.83} \\
            \bottomrule
            \end{tabular}
            }
      \end{center}
      %\vspace{-0.5cm}
      \caption{Comparison of our method to UDF \cite{DeLuigi23} on unseen shirts in resolution 256.
      }
      \label{tab:recon_unseen}
      %\vspace{-6mm}
      \vspace{-0.5cm}
  \end{table}
  

==> tabs/recon_unseen_pants.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
    \begin{center}
      \scalebox{1.}{
            \begin{tabular}{c | c | c}
            \toprule
             Trousers & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) \\
             \midrule
             UDF  & 0.425 & 98.09 \\
             \midrule
             Ours  & \textbf{0.346} & \textbf{98.32} \\
            \bottomrule
            \end{tabular}
            }
      \end{center}
      %\vspace{-0.5cm}
      \caption{Comparison of our method to UDF \cite{DeLuigi23} on unseen trousers in resolution 256.
      }
      \label{tab:recon_unseen_pants}
      %\vspace{-6mm}
      %\vspace{-0.5cm}
  \end{table}
  

==> tabs/recon_unseen_skirt.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%\begin{table}
%    \begin{center}
%      \scalebox{1.}{
%            \begin{tabular}{c | c | c}
%            \toprule
%             Skirt & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) \\
%             \midrule
%             UDF  & 0.403 & 98.64 \\
%             \midrule
%             Ours  & \textbf{0.362} & \textbf{98.85} \\
%            \bottomrule
%            \end{tabular}
%            }
%      \end{center}
%      %\vspace{-0.5cm}
%      \caption{Comparison of our method to UDF \cite{DeLuigi23} on unseen skirts in resolution 256.
%      }
%      \label{tab:recon_unseen_skirt}
%      %\vspace{-6mm}
%      %\vspace{-0.5cm}
%  \end{table}
\begin{table}[h!]
  \begin{center}
  \scalebox{0.75}{
    \begin{tabular}{c | c | c | c}
      \toprule
       Train & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) & Time (ms, $\downarrow$) \\
       \midrule
       UDF - 128  & 0.758 & 98.22 & 661 \\
       UDF - 256  & 0.430 & 98.56 & 2650 \\
       UDF - 512  & 0.342 & 98.33 & 17141 \\
       \midrule
       Ours - 128  & 0.545 & 98.28 & \textbf{25} \\
       Ours - 256  & 0.363 & 98.59 & 82 \\
       Ours - 512  & \textbf{0.317} & \textbf{98.62} & 269 \\
      \bottomrule
      \end{tabular}}
      ~~
  \scalebox{0.75}{
    \begin{tabular}{c | c | c}
      \toprule
       Test & CHD ($\times 10^{-4}$, $\downarrow$) & NC (\%, $\uparrow$) \\
       \midrule
       UDF - 128   & 0.752 & 97.41 \\
       UDF - 256   & 0.425 & 98.09 \\
       UDF - 512   & 0.350 & 97.63 \\
       \midrule
       Ours - 128   & 0.529 & 98.03 \\
       Ours - 256   & 0.346 & 98.31 \\
       Ours - 512   & \textbf{0.300} & \textbf{98.32} \\
      \bottomrule
      \end{tabular}
    }
  \end{center}
  \vspace{-1mm}
  \caption{Comparison of our method to UDF on trousers under the resolutions of 128, 256 and 512.}
  \label{tab:recon_pants}
\end{table}

==> tabs/traininng.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
    \begin{center}
      \scalebox{1.}{
            \begin{tabular}{c | c | c | c | c | c}
            \toprule
             Network & $\mathcal{I}_{\Theta}$ & $\mathcal{A}_{\Phi}$ & $w$ & $\mathcal{D}_s$ & $\mathcal{D}_m$ \\
             \midrule
             Learning Rate  & $10^{-4}$ & $10^{-4}$ & $10^{-4}$ & $5\times 10^{-5}$ & $10^{-4}$ \\
             Batch Size  & 50 & 50 & 6000 & 30 & 6\\
             Iterations  & 70000 & 70000 & 2000 & 20000 & 30000 \\
            \bottomrule
            \end{tabular}
            }
      \end{center}
      %\vspace{-0.5cm}
      \caption{Training hyperparameters.}
      \label{tab:training}
      %\vspace{-6mm}
      %\vspace{-0.5cm}
  \end{table}
  
